TraceSim: A Method for Calculating Stack Trace Similarity

Many contemporary software products have subsystems for automatic crash reporting. However, it is well-known that the same bug can produce slightly different reports. To manage this problem, reports are usually grouped, often manually by developers. Manual triaging, however, becomes infeasible for products that have large userbases, which is the reason for many different approaches to automating this task. Moreover, it is important to improve quality of triaging due to the big volume of reports that needs to be processed properly. Therefore, even a relatively small improvement could play a significant role in overall accuracy of report bucketing. The majority of existing studies use some kind of a stack trace similarity metric, either based on information retrieval techniques or string matching methods. However, it should be stressed that the quality of triaging is still insufficient. In this paper, we describe TraceSim -- a novel approach to address this problem which combines TF-IDF, Levenshtein distance, and machine learning to construct a similarity metric. Our metric has been implemented inside an industrial-grade report triaging system. The evaluation on a manually labeled dataset shows significantly better results compared to baseline approaches.

==> bibliography-long.tex <==
@inproceedings{Lerch:2013:FDY:2495256.2495763,
	author = {Lerch, Johannes and Mezini, Mira},
	title = {Finding Duplicates of Your Yet Unwritten Bug Report},
	booktitle = {Proceedings of the 2013 17th European Conference on Software Maintenance and Reengineering},
	series = {CSMR '13},
	year = {2013},
	isbn = {978-0-7695-4948-4},
	pages = {69--78},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/CSMR.2013.17},
	doi = {10.1109/CSMR.2013.17},
	acmid = {2495763},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {stack trace, duplicate detection, bug report},
} 

@inproceedings{Wu:2014:CLC:2610384.2610386,
	author = {Wu, Rongxin and Zhang, Hongyu and Cheung, Shing-Chi and Kim, Sunghun},
	title = {CrashLocator: Locating Crashing Faults Based on Crash Stacks},
	booktitle = {Proceedings of the 2014 International Symposium on Software Testing and Analysis},
	series = {ISSTA 2014},
	year = {2014},
	isbn = {978-1-4503-2645-2},
	location = {San Jose, CA, USA},
	pages = {204--214},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2610384.2610386},
	doi = {10.1145/2610384.2610386},
	acmid = {2610386},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Crashing fault localization, crash stack, software analytics, software crash, statistical debugging},
} 

@inproceedings{Campbell:2016:UET:2901739.2901766,
	author = {Campbell, Joshua Charles and Santos, Eddie Antonio and Hindle, Abram},
	title = {The Unreasonable Effectiveness of Traditional Information Retrieval in Crash Report Deduplication},
	booktitle = {Proceedings of the 13th International Conference on Mining Software Repositories},
	series = {MSR '16},
	year = {2016},
	isbn = {978-1-4503-4186-8},
	location = {Austin, Texas},
	pages = {269--280},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/2901739.2901766},
	doi = {10.1145/2901739.2901766},
	acmid = {2901766},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {automatic crash reporting, call stack trace, contextual information, deduplication, duplicate bug reports, duplicate crash report, free/open source software, information retrieval, software engineering},
} 

@INPROCEEDINGS{brodie,
	author={M. Brodie and Sheng Ma and G. Lohman and L. Mignet and N. Modani and M. Wilding and J. Champlin and P. Sohn},
	booktitle={Second International Conference on Autonomic Computing (ICAC'05)},
	title={Quickly Finding Known Software Problems via Automated Symptom Matching},
	year={2005},
	volume={},
	number={},
	pages={101-110},
	abstract={We present an architecture for and prototype of a system for quickly detecting software problem recurrences. Re-discovery of the same problem is very common in many large software products and is a major cost component of product support. At run-time, when a problem occurs, the system collects the problem symptoms, including the program call-stack, and compares it against a database of symptoms to find the closest matches. The database is populated off-line using solved cases and indexed to allow for efficient matching. Thus problems that occur repeatedly can be easily and automatically resolved without requiring any human problem-solving expertise. We describe a prototype implementation of the system, including the matching algorithm, and present some experimental results demonstrating the value of automatically detecting re-occurrence of the same problem for a popular sofware product},
	keywords={pattern matching;program debugging;program diagnostics;software engineering;automated symptom matching;system architecture;system prototype;software problem recurrence detection;software products;program call-stack;matching algorithm;Databases;Humans;Costs;Software systems;Computer architecture;Software prototyping;Runtime;Problem-solving;Prototypes;Measurement standards},
	doi={10.1109/ICAC.2005.49},
	ISSN={},
	month={June},}

@inproceedings{modani,
	author = {Modani, Natwar and Gupta, Rajeev and Lohman, Guy and Syeda-Mahmood, Tanveer and Mignet, Laurent},
	title = {Automatically Identifying Known Software Problems},
	booktitle = {Proceedings of the 2007 IEEE 23rd International Conference on Data Engineering Workshop},
	series = {ICDEW '07},
	year = {2007},
	isbn = {978-1-4244-0831-3},
	pages = {433--441},
	numpages = {9},
	url = {http://dx.doi.org/10.1109/ICDEW.2007.4401026},
	doi = {10.1109/ICDEW.2007.4401026},
	acmid = {1547620},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{bartz,
	author = {Bartz, Kevin and Stokes, Jack W. and Platt, John C. and Kivett, Ryan and Grant, David and Calinoiu, Silviu and Loihle, Gretchen},
	title = {Finding Similar Failures Using Callstack Similarity},
	booktitle = {Proceedings of the Third Conference on Tackling Computer Systems Problems with Machine Learning Techniques},
	series = {SysML'08},
	year = {2008},
	location = {San Diego, California},
	pages = {1--1},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=1855895.1855896},
	acmid = {1855896},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
} 

@inproceedings{dang,
	author = {Dang, Yingnong and Wu, Rongxin and Zhang, Hongyu and Zhang, Dongmei and Nobel, Peter},
	title = {ReBucket: A Method for Clustering Duplicate Crash Reports Based on Call Stack Similarity},
	booktitle = {Proceedings of the 34th International Conference on Software Engineering},
	series = {ICSE '12},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {1084--1093},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337364},
	acmid = {2337364},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@inproceedings{dhaliwal,
	author = {Dhaliwal, Tejinder and Khomh, Foutse and Zou, Ying},
	title = {Classifying Field Crash Reports for Fixing Bugs: A Case Study of Mozilla Firefox},
	booktitle = {Proceedings of the 2011 27th IEEE International Conference on Software Maintenance},
	series = {ICSM '11},
	year = {2011},
	isbn = {978-1-4577-0663-9},
	pages = {333--342},
	numpages = {10},
	url = {https://doi.org/10.1109/ICSM.2011.6080800},
	doi = {10.1109/ICSM.2011.6080800},
	acmid = {2119726},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{levenshtein,
	author = {Levenshtein, V. I.},
	journal = {Soviet Physics Doklady},
	pages = {707--710},
	title = {Binary Codes Capable of Correcting Deletions, Insertions and Reversals},
	volume = 10,
	year = 1966
}

@inproceedings{lerch,
	author = {Lerch, Johannes and Mezini, Mira},
	title = {Finding Duplicates of Your Yet Unwritten Bug Report},
	booktitle = {Proceedings of the 2013 17th European Conference on Software Maintenance and Reengineering},
	series = {CSMR '13},
	year = {2013},
	isbn = {978-0-7695-4948-4},
	pages = {69--78},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/CSMR.2013.17},
	doi = {10.1109/CSMR.2013.17},
	acmid = {2495763},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {stack trace, duplicate detection, bug report},
} 

@INPROCEEDINGS{schroter,
	author={A. Schroter and A. Schröter and N. Bettenburg and R. Premraj},
	booktitle={2010 7th IEEE Working Conference on Mining Software Repositories (MSR 2010)},
	title={Do stack traces help developers fix bugs?},
	year={2010},
	volume={},
	number={},
	pages={118-121},
	abstract={A widely shared belief in the software engineering community is that stack traces are much sought after by developers to support them in debugging. But limited empirical evidence is available to confirm the value of stack traces to developers. In this paper, we seek to provide such evidence by conducting an empirical study on the usage of stack traces by developers from the ECLIPSE project. Our results provide strong evidence to this effect and also throws light on some of the patterns in bug fixing using stack traces. We expect the findings of our study to further emphasize the importance of adding stack traces to bug reports and that in the future, software vendors will provide more support in their products to help general users make such information available when filing bug reports.},
	keywords={program debugging;software engineering;stack traces;software engineering;debugging;ECLIPSE project;bug fixing;Computer bugs;Software engineering;Collaboration;Programming profession;Software debugging;Needles;Open source software;Computer crashes;Documentation;Java;debugging;stack traces;empirical study;bug tracking;collaboration},
	doi={10.1109/MSR.2010.5463280},
	ISSN={2160-1852},
	month={May},}

@inproceedings{microsoft,
	author = {Glerum, Kirk and Kinshumann, Kinshuman and Greenberg, Steve and Aul, Gabriel and Orgovan, Vince and Nichols, Greg and Grant, David and Loihle, Gretchen and Hunt, Galen},
	title = {Debugging in the (Very) Large: Ten Years of Implementation and Experience},
	booktitle = {Proceedings of the ACM SIGOPS 22Nd Symposium on Operating Systems Principles},
	series = {SOSP '09},
	year = {2009},
	isbn = {978-1-60558-752-3},
	location = {Big Sky, Montana, USA},
	pages = {103--116},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1629575.1629586},
	doi = {10.1145/1629575.1629586},
	acmid = {1629586},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {blue screen of death, bucketing, classifying, error reports, labeling, minidump, statistics-based debugging.},
} 

@article{NEEDLEMAN1970443,
	title = "A general method applicable to the search for similarities in the amino acid sequence of two proteins",
	journal = "Journal of Molecular Biology",
	volume = "48",
	number = "3",
	pages = "443--453",
	year = "1970",
	issn = "0022-2836",
	doi = "https://doi.org/10.1016/0022-2836(70)90057-4",
	url = "http://www.sciencedirect.com/science/article/pii/0022283670900574",
	author = "Saul B. Needleman and Christian D. Wunsch",
	abstract = "A computer adaptable method for finding similarities in the amino acid sequences of two proteins has been developed. From these findings it is possible to determine whether significant homology exists between the proteins. This information is used to trace their possible evolutionary development. The maximum match is a number dependent upon the similarity of the sequences. One of its definitions is the largest number of amino acids of one protein that can be matched with those of a second protein allowing for all possible interruptions in either of the sequences. While the interruptions give rise to a very large number of comparisons, the method efficiently excludes from consideration those comparisons that cannot contribute to the maximum match. Comparisons are made from the smallest unit of significance, a pair of amino acids, one from each protein. All possible pairs are represented by a two-dimensional array, and all possible comparisons are represented by pathways through the array. For this maximum match only certain of the possible pathways must be evaluated. A numerical value, one in this case, is assigned to every cell in the array representing like amino acids. The maximum match is the largest number that would result from summing the cell values of every pathway."
}

@inproceedings{Wang:2013:IBL:2487085.2487135,
	author = {Wang, Shaohua and Khomh, Foutse and Zou, Ying},
	title = {Improving Bug Localization Using Correlations in Crash Reports},
	booktitle = {Proceedings of the 10th Working Conference on Mining Software Repositories},
	series = {MSR '13},
	year = {2013},
	isbn = {978-1-4673-2936-1},
	location = {San Francisco, CA, USA},
	pages = {247--256},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=2487085.2487135},
	acmid = {2487135},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@INPROCEEDINGS{Cubranic04automaticbug,
	author = {Davor Čubranić},
	title = {Automatic bug triage using text categorization},
	booktitle = {In SEKE 2004: Proceedings of the Sixteenth International Conference on Software Engineering & Knowledge Engineering},
	year = {2004},
	pages = {92--97},
	publisher = {KSI Press}
}

@article{Knuth1977,
  doi = {10.1137/0206024},
  url = {https://doi.org/10.1137/0206024},
  year  = {1977},
  month = {jun},
  publisher = {Society for Industrial {\&} Applied Mathematics ({SIAM})},
  volume = {6},
  number = {2},
  pages = {323--350},
  author = {Donald E. Knuth and James H. Morris,  Jr. and Vaughan R. Pratt},
  title = {Fast Pattern Matching in Strings},
  journal = {{SIAM} Journal on Computing}
}

@article{sparck1972statistical,
	title={A statistical interpretation of term specificity and its application in retrieval},
	author={Sparck Jones, Karen},
	journal={Journal of documentation},
	volume={28},
	number={1},
	pages={11--21},
	year={1972},
	publisher={MCB UP Ltd}
}

@article{claesen2015hyperparameter,
	title={Hyperparameter search in machine learning},
	author={Claesen, Marc and De Moor, Bart},
	journal={arXiv preprint arXiv:1502.02127},
	year={2015}
}

@inproceedings{bergstra2013hyperopt,
	title={Hyperopt: A python library for optimizing the hyperparameters of machine learning algorithms},
	author={Bergstra, James and Yamins, Dan and Cox, David D},
	booktitle={Proceedings of the 12th Python in Science Conference},
	pages={13--20},
	year={2013},
	organization={Citeseer}
}

@article{Navarro2001,
	doi = {10.1145/375360.375365},
	url = {https://doi.org/10.1145/375360.375365},
	year  = {2001},
	month = {mar},
	publisher = {Association for Computing Machinery ({ACM})},
	volume = {33},
	number = {1},
	pages = {31--88},
	author = {Gonzalo Navarro},
	title = {A guided tour to approximate string matching},
	journal = {{ACM} Computing Surveys}
}

@article{Fawcett2006,
  doi = {10.1016/j.patrec.2005.10.010},
  url = {https://doi.org/10.1016/j.patrec.2005.10.010},
  year  = {2006},
  month = {jun},
  publisher = {Elsevier {BV}},
  volume = {27},
  number = {8},
  pages = {861--874},
  author = {Tom Fawcett},
  title = {An introduction to {ROC} analysis},
  journal = {Pattern Recognition Letters}
}

@inproceedings{Koopaei:2015:CAD:2886444.2886474,
	author = {Koopaei, Neda Ebrahimi and Hamou-Lhadj, Abdelwahab},
	title = {CrashAutomata: An Approach for the Detection of Duplicate Crash Reports Based on Generalizable Automata},
	booktitle = {Proceedings of the 25th Annual International Conference on Computer Science and Software Engineering},
	series = {CASCON '15},
	year = {2015},
	location = {Markham, Canada},
	pages = {201--210},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=2886444.2886474},
	acmid = {2886474},
	publisher = {IBM Corp.},
	address = {Riverton, NJ, USA},
	keywords = {automata-based modeling, duplicate bug reports, mining bug repositories, software maintenance},
} 

@inproceedings{K.:2016:EMD:3049877.3049885,
	author = {K., Neda Ebrahimi and Islam, Md. Shariful and Hamou-Lhadj, Abdelwahab and Hamdaqa, Mohammad},
	title = {An Effective Method for Detecting Duplicate Crash Reports Using Crash Traces and Hidden Markov Models},
	booktitle = {Proceedings of the 26th Annual International Conference on Computer Science and Software Engineering},
	series = {CASCON '16},
	year = {2016},
	location = {Toronto, Ontario, Canada},
	pages = {75--84},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=3049877.3049885},
	acmid = {3049885},
	publisher = {IBM Corp.},
	address = {Riverton, NJ, USA},
	keywords = {hidden markov model, mining bug repositories duplicate crash reports, software maintenance},
} 

@INPROCEEDINGS{5958261,
	author={S. Kim and T. Zimmermann and N. Nagappan},
	booktitle={2011 IEEE/IFIP 41st International Conference on Dependable Systems Networks (DSN)},
	title={Crash graphs: An aggregated view of multiple crashes to improve crash triage},
	year={2011},
	volume={},
	number={},
	pages={486-493},
	keywords={graph theory;program debugging;software reliability;system recovery;crash graphs;crash triage;crash reporting systems;system reliability;system dependability;Windows error reporting system;debugging;Computer bugs;Debugging;Servers;Algorithm design and analysis;Feature extraction;Complexity theory;crash;graph;triaging;network},
	doi={10.1109/DSN.2011.5958261},
	ISSN={2158-3927},
	month={June},}

@Article{Hindle2018,
	author="Hindle, Abram
	and Onuczko, Curtis",
	title="Preventing duplicate bug reports by continuously querying bug reports",
	journal="Empirical Software Engineering",
	year="2018",
	month="Aug",
	day="20",
	abstract="Bug deduplication or duplicate bug report detection is a hot topic in software engineering information retrieval research, but it is often not deployed. Typically to de-duplicate bug reports developers rely upon the search capabilities of the bug report software they employ, such as Bugzilla, Jira, or Github Issues. These search capabilities range from simple SQL string search to IR-based word indexing methods employed by search engines. Yet too often these searches do very little to stop the creation of duplicate bug reports. Some bug trackers have more than 10{\%} of their bug reports marked as duplicate. Perhaps these bug tracker search engines are not enough? In this paper we propose a method of attempting to prevent duplicate bug reports before they start: continuously querying. That is as the bug reporter types in their bug report their text is used to query the bug database to find duplicate or related bug reports. This continuously querying bug reports allows the reporter to be alerted to duplicate bug reports as they report the bug, rather than formulating queries to find the duplicate bug report. Thus this work ushers in a new way of evaluating bug report deduplication techniques, as well as a new kind of bug deduplication task. We show that simple IR measures can address this problem but also that further research is needed to refine this novel process that is integrate-able into modern bug report systems.",
	issn="1573-7616",
	doi="10.1007/s10664-018-9643-4",
	url="https://doi.org/10.1007/s10664-018-9643-4"
}

@ARTICLE{8048025,
	author={M. S. Rakha and C. Bezemer and A. E. Hassan},
	journal={IEEE Transactions on Software Engineering},
	title={Revisiting the Performance Evaluation of Automated Approaches for the Retrieval of Duplicate Issue Reports},
	year={2018},
	volume={44},
	number={12},
	pages={1245-1268},
	keywords={Text analysis;Computer bugs;Frequency measurement;Performance evaluation;Manuals;Ports (Computers);Text analysis;software engineering;performance evaluation},
	doi={10.1109/TSE.2017.2755005},
	ISSN={0098-5589},
	month={Dec},}

@INPROCEEDINGS{6100061,
	author={C. Sun and D. Lo and S. Khoo and J. Jiang},
	booktitle={2011 26th IEEE/ACM International Conference on Automated Software Engineering (ASE 2011)},
	title={Towards more accurate retrieval of duplicate bug reports},
	year={2011},
	volume={},
	number={},
	pages={253-262},
	keywords={gradient methods;information retrieval;learning (artificial intelligence);program debugging;bug tracking system;duplicate bug reports;retrieval function;textual similarity;BM25F;information retrieval community;duplicate report retrieval;two-round stochastic gradient descent;REP;supervised learning;software bug repositories;Training;Accuracy;Computer bugs;Tuning;Information retrieval;Support vector machines;Software},
	doi={10.1109/ASE.2011.6100061},
	ISSN={1938-4300},
	month={Nov},}

@book{Manning:2008:IIR:1394399,
	author = {Manning, Christopher D. and Raghavan, Prabhakar and Sch\"{u}tze, Hinrich},
	title = {Introduction to Information Retrieval},
	year = {2008},
	isbn = {0521865719, 9780521865715},
	publisher = {Cambridge University Press},
	address = {New York, NY, USA},
} 

@inproceedings{Glerum:2009:DLT:1629575.1629586,
	author = {Glerum, Kirk and Kinshumann, Kinshuman and Greenberg, Steve and Aul, Gabriel and Orgovan, Vince and Nichols, Greg and Grant, David and Loihle, Gretchen and Hunt, Galen},
	title = {Debugging in the (Very) Large: Ten Years of Implementation and Experience},
	booktitle = {Proceedings of the ACM SIGOPS 22Nd Symposium on Operating Systems Principles},
	series = {SOSP '09},
	year = {2009},
	isbn = {978-1-60558-752-3},
	location = {Big Sky, Montana, USA},
	pages = {103--116},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1629575.1629586},
	doi = {10.1145/1629575.1629586},
	acmid = {1629586},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {blue screen of death, bucketing, classifying, error reports, labeling, minidump, statistics-based debugging.},
} 

@misc{Sam007:periododic,
	author = {Sumit Sudhakar, and Harshit Agrawal},
	title = {Find if a given string can be represented from a substring by iterating the substring n times},
	howpublished = "\url{https://www.geeksforgeeks.org/find-given-string-can-represented-substring-iterating-substring-n-times}",
	note = "[Online; accessed 20-January-2019]"
}

@Inbook{Apostolico1997,
	author="Apostolico, Alberto
	and Breslauer, Dany",
	editor="Mycielski, Jan
	and Rozenberg, Grzegorz
	and Salomaa, Arto",
	title="Of periods, quasiperiods, repetitions and covers",
	bookTitle="Structures in Logic and Computer Science: A Selection of Essays in Honor of A. Ehrenfeucht",
	year="1997",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="236--248",
	abstract="Quasiperiodic strings were defined by Apostolico and Ehrenfeucht [3], as strings which are entirly covered by occurrences of another(shorter) string. This paper surveys a handful of results on the structure and detection of quasiperiodic strings and on related string covers,attempting to simplify and present in a uniform manner the algorithms being surveyed.",
	isbn="978-3-540-69242-3",
	doi="10.1007/3-540-63246-8_14",
	url="https://doi.org/10.1007/3-540-63246-8_14"
}

@article{newman2005power,
	title={{Power laws, Pareto distributions and Zipf's law}},
	author={Newman, Mark EJ},
	journal={Contemporary physics},
	volume={46},
	number={5},
	pages={323--351},
	year={2005},
	publisher={Taylor \& Francis}
}

@inproceedings{Ling:2003:ASC:1630659.1630736,
	author = {Ling, Charles X. and Huang, Jin and Zhang, Harry},
	title = {AUC: A Statistically Consistent and More Discriminating Measure Than Accuracy},
	booktitle = {Proceedings of the 18th International Joint Conference on Artificial Intelligence},
	series = {IJCAI'03},
	year = {2003},
	location = {Acapulco, Mexico},
	pages = {519--524},
	numpages = {6},
	url = {http://dl.acm.org/citation.cfm?id=1630659.1630736},
	acmid = {1630736},
	publisher = {Morgan Kaufmann Publishers Inc.},
	address = {San Francisco, CA, USA},
} 

@article{ROC,
	author = {Liu, Honghu and Li, Gang and Cumberland, William and Wu, Tongtong},
	year = {2005},
	month = {01},
	pages = {257--278},
	title = {Testing Statistical Significance of the Area under a Receiving Operating Characteristics Curve for Repeated Measures Design with Bootstrapping},
	volume = {3},
	journal = {Journal of Data Science}
}

@article{10.2307/2958830,
	ISSN = {00905364},
	URL = {http://www.jstor.org/stable/2958830},
	abstract = {We discuss the following problem: given a random sample X = (X1, X2, ⋯, Xn) from an unknown probability distribution F, estimate the sampling distribution of some prespecified random variable R(X, F), on the basis of the observed data x. (Standard jackknife theory gives an approximate mean and variance in the case R(X, F) = θ(F̂) - θ(F), θ some parameter of interest.) A general method, called the "bootstrap," is introduced, and shown to work satisfactorily on a variety of estimation problems. The jackknife is shown to be a linear approximation method for the bootstrap. The exposition proceeds by a series of examples: variance of the sample median, error rates in a linear discriminant analysis, ratio estimation, estimating regression parameters, etc.},
	author = {B. Efron},
	journal = {The Annals of Statistics},
	number = {1},
	pages = {1--26},
	publisher = {Institute of Mathematical Statistics},
	title = {Bootstrap Methods: Another Look at the Jackknife},
	volume = {7},
	year = {1979}
}

@INPROCEEDINGS{7866753,
	author={M. A. {Ghafoor} and J. H. {Siddiqui}},
	booktitle={2016 International Conference on Frontiers of Information Technology (FIT)},
	title={Cross Platform Bug Correlation Using Stack Traces},
	year={2016},
	volume={},
	number={},
	pages={199-204},
	keywords={program debugging;software fault tolerance;cross platform bug correlation;stack traces;program crashing;event log;crash reporting programs;faulty function detection;function call stack;bug reports;similarity metric;Computer bugs;Measurement;Correlation;Data mining;Software;Libraries;Bug reports;Stack traces},
	doi={10.1109/FIT.2016.044},
	ISSN={},
	month={Dec},}

@misc{Elasticsearch,
  title = {Elasticsearch},
  howpublished = {\url{https://www.elastic.co/products/elasticsearch}},
  note = {Accessed: {2019-11-08}}
}

@misc{RebucketImplementation,
  title = {Implementation of {R}ebucket},
  howpublished = {\url{https://github.com/ZhangShurong/rebucket}},
  note = {Accessed: {2019-11-08}}
}

@misc{Hyperopt,
  title = {Hyperopt},
  howpublished = {\url{https://github.com/hyperopt/hyperopt}},
  note = {Accessed: {2019-11-08}}
}

@misc{TraceSim,
  title = {Trace{S}im implementation},
  howpublished = {\url{https://github.com/traceSimSubmission/trace-sim}},
  note = {Accessed: {2019-11-08}}
}

@inproceedings{10.5555/3042817.3042832,
author = {Bergstra, J. and Yamins, D. and Cox, D. D.},
title = {Making a Science of Model Search: Hyperparameter Optimization in Hundreds of Dimensions for Vision Architectures},
year = {2013},
publisher = {JMLR.org},
booktitle = {Proceedings of the 30th International Conference on International Conference on Machine Learning - Volume 28},
pages = {I–115–I–123},
numpages = {9},
location = {Atlanta, GA, USA},
series = {ICML’13}
}

@inproceedings{10.5555/2986459.2986743,
author = {Bergstra, James and Bardenet, R\'{e}mi and Bengio, Yoshua and K\'{e}gl, Bal\'{a}zs},
title = {Algorithms for Hyper-Parameter Optimization},
year = {2011},
isbn = {9781618395993},
publisher = {Curran Associates Inc.},
address = {Red Hook, NY, USA},
booktitle = {Proceedings of the 24th International Conference on Neural Information Processing Systems},
pages = {2546–2554},
numpages = {9},
location = {Granada, Spain},
series = {NIPS’11}
}

@inproceedings{DBLP:conf/seke/MorooAH17,
  author    = {Akira Moroo and
               Akiko Aizawa and
               Takayuki Hamamoto},
  editor    = {Xudong He},
  title     = {Reranking-based Crash Report Deduplication},
  booktitle = {The 29th International Conference on Software Engineering and Knowledge
               Engineering, Wyndham Pittsburgh University Center, Pittsburgh, PA,
               USA, July 5-7, 2017},
  pages     = {507--510},
  publisher = {{KSI} Research Inc. and Knowledge Systems Institute Graduate School},
  year      = {2017},
  url       = {https://doi.org/10.18293/SEKE2017-135},
  doi       = {10.18293/SEKE2017-135},
  timestamp = {Thu, 12 Mar 2020 11:30:50 +0100},
  biburl    = {https://dblp.org/rec/conf/seke/MorooAH17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@INPROCEEDINGS{8009929,
author={K. K. {Sabor} and A. {Hamou-Lhadj} and A. {Larsson}},
booktitle={2017 IEEE International Conference on Software Quality, Reliability and Security (QRS)}, 
title={DURFEX: A Feature Extraction Technique for Efficient Detection of Duplicate Bug Reports}, 
year={2017},
volume={},
number={},
pages={240-250},
}

@article{10.1007/s10664-018-9643-4,
author = {Hindle, Abram and Onuczko, Curtis},
title = {Preventing Duplicate Bug Reports by Continuously Querying Bug Reports},
year = {2019},
issue_date = {April     2019},
publisher = {Kluwer Academic Publishers},
address = {USA},
volume = {24},
number = {2},
issn = {1382-3256},
url = {https://doi.org/10.1007/s10664-018-9643-4},
doi = {10.1007/s10664-018-9643-4},
journal = {Empirical Softw. Engg.},
month = apr,
pages = {902–936},
numpages = {35},
keywords = {Issue reports, Deduplication, Information retrieval, Continuously querying bug reports, Duplicate bug reports, Continuous query, Just in time}
}

==> empstudy.tex <==
\label{sec:empstudy}

% TODO: маловато будет, несколько миллионов :( -> исчисляется миллионами, 2000 в день; мы привыкли получать тысячи репортов в день.

Exception Analyzer and the workflow described above have been used inside the company since the early 00's. Currently, several millions of reports have been collected for the IntelliJ Platform. In this section, we present a study of this data, in which we assess the properties of the existing bucketing algorithm and the usefulness of the resulting buckets. For these purposes, we have run a series of exploratory experiments on a subset of our database that includes all reports from 2017 to 2018.


\begin{figure*}
	\center
	\begin{minipage}[b]{0.49\textwidth}
		\includegraphics[width=\textwidth]{./figures/issues_by_size_all.png}
		\subcaption{Distribution of reports in issues, top issues}
		\label{fig:issuesize15}		
	\end{minipage}
	\begin{minipage}[b]{0.49\textwidth}
	\includegraphics[width=\textwidth]{./figures/issue_count_all.png}
	\subcaption{Distribution of issue sizes, all}
	\label{fig:issuesizeall}
	\end{minipage}
	\begin{minipage}[b]{0.49\textwidth}
		\includegraphics[width=\textwidth]{./figures/issues_size_all.png}
		\subcaption{Distribution of reports in issues, all}
		\label{fig:reportdistrib}
	\end{minipage}
	\begin{minipage}[b]{0.49\textwidth}
		\includegraphics[width=\textwidth]{./figures/issues_fix_prob_all.png}
		\subcaption{Issue fix probability}
		\label{fig:issfixidea}
	\end{minipage}
	\caption{Empirical study results}
\end{figure*}

\subsection{Distribution of issues sizes: long tail}\label{sec:empissuesize}

Figure~\ref{fig:issuesize15} shows the distribution of issues according to the number of contained reports in IntelliJ Platform products. On this diagram, blue bars indicate the number of reports in top $15$ issues, normalized by the largest issue. Each of the yellow bars represents the share of all reports that is contained in all previous issues, including the current one. This way: 
\begin{itemize}
	\item the first yellow bar shows how many reports (out of all stored) belong to the first bucket,
	\item the last yellow bar indicates that top $15$ issues (by size) contain roughly $20$\% of all stored reports.
\end{itemize}

Next, Figures~\ref{fig:issuesizeall}, \ref{fig:reportdistrib} show the properties of issue distribution at large. These graphs were constructed using the same procedure. The idea is to assign each issue to a single bucket as follows:

\begin{enumerate}
	\item For each issue $i$ we calculate 
	
	$$r = \frac{\log (\text{Number of reports in } i)} {\log(\text{Maximum number of reports in issue})}$$
	
	\item The result would belong to the $[0, 1]$ range, which we divide into $10$ buckets as follows: $[0, 0.1), [0.1, 0.2), \ldots [0.9, 1]$. We assign $i$ to the bucket which contains $r$.
	\item Finally, for each bucket we calculate some statistic using only contained issues.
\end{enumerate}

Designing this procedure, we were motivated by the fact that in our database, issue sizes are distributed in a skewed manner: there are many more small issues than large ones. Therefore, we had to resort to logarithmization and bucketing in order to construct a readable view of the Exception Analyzer database. 

Informally, one may say that on these plots issues that have the smallest number of reports are placed to the left. Thereby, the size of issues increases while moving along the X-axis to the right. Note that as the result of the first step the axis becomes logarithmic. 

Let us start with the assessment of the resulting buckets. Figure~\ref{fig:issuesizeall} shows the number of issues that fell into a particular bucket i.e., it plots the number of issues against issue size. This bar chart shows that small issues constitute the majority and comprise more than 80\% of the whole database. This and the next graph demonstrate the presence of a ``long tail'' problem in our report database, similarly to WER~\cite{dang}.

For Figure~\ref{fig:reportdistrib}, the total number of reports inside each bucket (over all issues) was counted. Therefore, this bar chart shows the overall share of reports that is contributed by a group of issues that have an approximately equal number of reports. Together with the previous figure it demonstrates that the majority of reports are contained in medium-sized issues. At the same time, a small number of the largest issues (belonging to two rightmost buckets) contribute approximately the same number of reports as the four leftmost buckets.

\subsection{Issue size and fix probability}\label{sec:empsizefixprob}

Figure~\ref{fig:issfixidea} describes the probability of being fixed for a particular issue depending on the number of contained reports. This bar chart is constructed similarly to the previous ones, but at the last step, the ratio of fixed issues was calculated. We can see that issues having the largest number of reports (rightmost column) have the lowest number of fixed issues. The other interesting region is the set of leftmost columns. We can see that the smallest issues are also fixed infrequently compared to the ``central'' ones, which have the maximum probability. In overall, it is possible to say that the following regularity is present: issues having a medium number of issues have increased fix probability compared to the corner ones. Only the second bucket from the right sticks out: all of its issues are fixed. However, it is an outlier because the two rightmost buckets have less than a dozen of issues due to the nature of issue distribution. The same dependency was indicated in a study by Dang et al. results~\cite{dang}.


% вообще, идея на будущее: статья про время жизни репортов/issue и другие метрики, в зависимости от стадии "зрелости" продукта

% TODO: всё-таки надо побольше объяснений почему справа фиксится быстро

\subsection{Recursion and its influence on bucketing}\label{sec:emprecursion}

We have decided to start with the estimation of how frequently recursion appears in our report database. For this, we have decided to consider a standard Java exception ``java.util.StackOverflowError'' that is thrown when an execution thread runs out of the available stack space. It is a strong evidence of recursion presence, since in this case the stack size may contain several thousands of frames and this usually means that the same function (or a group of functions) appear multiple times. In the Exception Analyzer database, such reports constituted $2.8$\% of all reports that were generated during the two-year period.

Next, we have studied an average number of frames in stack traces with this exception. There are two reasons for this number to be of interest:
\begin{enumerate}
	\item it should be sufficiently large to have a noticeable impact on the performance of recursion elimination algorithm;
	\item it varies considerably since it depends on JVM settings, size, and number of local variables in the recursion code.
\end{enumerate}

Exploring our database, we have learned the following: the average stack trace size is $8570$ frames over a $1000$ of randomly-sampled reports containing ``java.util.StackOverflowError'' exception.

\subsection{Discussion}\label{sec:empconclusion}

Dang et al.~\cite{dang} indicated that there are two main problems with bucketing in crash report databases: a large number of issues containing a few reports (long tail problem), and reports, belonging to one bug, being spread around several issues (second bucket problem). Our empirical study demonstrated that these problems exist in Exception Analyzer database too.

Next, Dang et al. argued that the quality of bucketing affects bug fixing speed. Our empirical study demonstrated that this is indeed true: Figure~\ref{fig:issfixidea} shows that there is a direct link between issue size and fix probability. 

It can be explained as follows. Programmers employ these databases during effort prioritization and problem diagnostic. Small issues contain too few reports to provide enough information for a fix, or, at the same time, they are of a low priority since they affect smaller number of use-cases. Largest issues are fixed rarely due to either being junk issues that acquired this number of reports due to incorrect bucketing, or due to being a long-standing architectural problem that is hard to fix.

Aside from being useless for programmers, junk issues tend to grow by absorbing lots of incoming reports, which do not belong to this issue. Thus, their existence aggravates second bucket problem.

The similarity function plays a vital role in the automatic bucketing process and directly impacts the properties of generated issues: their number and sizes, their distribution. Similarity that produces a lot of Type I errors will lead to large and meaningless issues. At the same time Type II errors will lead to a large number of small issues that should have been merged. Therefore, improvement of bucketing accuracy may increase productivity of crash report system users. 

Next, during bucketing, similarity calculation function would be invoked multiple times. It is well-known~\cite{brodie, modani} that recursion not only slows down calculation, but reduces the quality of bucketing too. Our empirical study have demonstrated the need for algorithms having low computational complexity, since recursion-containing stack traces may span several thousands of frames and there is a significant amount of them.

We can conclude with the following: the quality of the bucketing algorithm that is currently in use in our company not sufficient. Moreover, the problem of bucketing quality was raised by many other studies that involved other datasets and algorithms~\cite{dang, Campbell:2016:UET:2901739.2901766}. It is an important issue since the quality seriously impacts the usefulness of the crash report management systems. 

==> excess.tex <==
% То, что не вошло в статью но пригодится для журнальной версии
The problem of automatic bug report deduplication is rather old. However, its formulation has evolved over time. Initially, the research community concentrated on deduplication of reports that consisted of a user-written textual description of a bug, and possibly other provided information such as tags, categories, and severity. In this paper, we do not concentrate on this type of studies, although some of them are listed in references~\cite{Hindle2018,8048025,6100061}. Note that early studies imply manual filling of bug report forms.

Later, the community's focus shifted to generated reports and researchers started to consider stack traces as well. This shift was driven by the fact that systems for automatic collection of generated reports were widely adopted by the industy. Therefore, in recent studies, the formulation deals with a steady stream of generated crash reports that contain only stack traces. 

There are two major approaches for triaging reports that use stack traces: pairwise similarity-based and model-based. In the former, stack traces are compared with each other and then similar ones are grouped into buckets. The latter proposes a procedure which takes a report (or a number of reports) and then assigns it to a bucket or generates a bucket out of them. The procedure does not feature an explicit similarity function and is usually implemented with some kind of machine learning approach. References~\cite{Koopaei:2015:CAD:2886444.2886474, K.:2016:EMD:3049877.3049885, 5958261} can serve as examples of model-based studies.

Currently, the pairwise similarity-based approach is more popular. Its basic methods include~\cite{modani}: Longest Common Subsequence, Prefix Match and Edit Distance. They are frequently used as a baseline for comparison.

%%%%%%%%%%%%%%%%%%%%%%%%

Recursion is frequently encountered in stack traces. It is believed that stack traces with recursion not only require additional computational resources to handle, but also negatively impact the quality of matching. Therefore, it is usually eliminated from stack traces using a special algorithm.

%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
The overall picture is presented in Table~\ref{tbl:classification}. Let us now briefly describe these studies.

A study by Brodie et al.~\cite{brodie} was one of the earliest that addressed the problem of crash report deduplication using stack trace comparison. It features removal of common uninformative functions, recursion elimination, and an indexing scheme.

The authors argue that biological sequence searching algorithms are more suitable for the considered problem than string matching ones. This is claimed due to the following: 
\begin{itemize}
\item in stack traces gaps of functions are more common than function substitutions;
\item the position of matching functions is very important; it is necessary to give functions on the top of the stack trace more weight.
\end{itemize}

For these reasons, a modification of the Needleman-Wunsch algorithm~\cite{NEEDLEMAN1970443} was proposed.

% GEORGE: можно ли считать prefix match каким-то подвидом сигнатурного метода? обобщить?
The authors of~\cite{modani} provide a comparison of three methods for calculating stack trace similarity. They compare the performance of the edit distance approach with prefix match and Longest Common Subsequence (LCS).

To improve the quality and run times of these methods, several modifications were evaluated: 1) recursion elimination, 2) uninformative function elimination, 3) several methods of indexing.

Experiments demonstrated the superiority of prefix approach in terms of precision. In turn, edit distance as well as LCS were able to attain higher levels of recall.

Bartz et al.~\cite{bartz} consider a slightly different problem~--- failure deduplication. In their case, any trouble with an application is detected by a special process that monitors the target process. Therefore, a crash report is only a part of the obtained telemetry data. This approach allows to detect not only crashes, but a broader range of issues, for example, deadlocks or hangs.

To perform deduplication of program failures, the authors build a failure similarity classifier. Essentially, it is a linear logistic probability model which has three simple binary categorical features (for example, same or different process names) and a non-binary callstack similarity. 

For the latter, a modification of edit distance metric is proposed. The authors introduce a notion of frame group: a consecutive group of frames in a callstack that belong to the same module. This leads to a number of operations, that should be differently scored. For example, inserting a new frame group should be penalized more than inserting a new frame into an existing frame group. In overall, seven edit operations with different weights were proposed.

The study~\cite{dhaliwal} describes the approach that combines signatures and Levenshtein distance between stack traces to calculate stack trace similarity. The proposed two-step approach is the following: first, reports are grouped together using only the first frame. Then, each bucket is split into several subgroups using the Levenshtein distance between stack traces (only the top 10 frames are used). 

To speed up calculations, a representative trace of each subgroup is computed. This trace is an array of sets~--- one for each of the top 10 frames of the stack traces that belong to the subgroup. Each set enumerates modules and their number of occurrence in the respective frame.

To compare a candidate stack trace with a representative one, Levenshtein distance is used as well. However, since they are different types of objects, the authors construct a function for distance calculation between their elements. Based on the resulting Levenshtein distance, a candidate stack trace is either attached to an existing subgroup or a new subgroup is created for the corresponding crash-report.

The Crash Graph~\cite{5958261} can also be thought of as a pairwise similarity-based approach, since, technically, it can be used to measure similarity of two stack traces. The core of the approach is the following: using stack traces contained in a bucket, build a special graph, then apply a graph similarity measure to decide whether the new stack trace belongs to this bucket. The graph is constructed by incrementally adding edges of all stack traces, where each edge is a pair of consequently encountered frames.

In~\cite{dang}, a novel bucketing approach and the crash stack similarity metric are discussed. The metric is based on the following parameters:
\begin{enumerate}
\item the offset distance between the matched functions;
\item the distance of these functions to the top frame.
\end{enumerate}

The authors show that this metric can be computed by an algorithm similar to one used to compute the LCS metric. Using this similarity function, an Agglomerative Hierarchical clustering is performed. Experiments have demonstrated the superiority over Crash Graph approach, WER bucketing~\cite{Glerum:2009:DLT:1629575.1629586}, and prefix match.

The study~\cite{Wang:2013:IBL:2487085.2487135} explores the relations between generated buckets. The authors study correlated buckets~--- buckets that correspond to identical or correlated bugs. In its turn, a correlated crash is a crash the occurrence of which causes the other crash to occur.

The primary goal of this study was the identification of correlated buckets. For this purpose, the authors have proposed three rules: crash signature comparison, top frame comparison, and frequent closed ordered sub-set comparison. The first one checks for containment of crash signatures according to the proposed definition. The second one checks whether the top frames are matching. The last rule is an adaptation of frequent item set mining for a set of stack frames.

%It is necessary to note that in the considered datasets bucketing was performed via signature method, i.e. if top frames of crash reports match, then, they go to a single bucket. -- TODO, подумать


In reference~\cite{Lerch:2013:FDY:2495256.2495763}, the authors study the situation when a bug tracker does not contain a dedicated field for storing crash stacks. In such cases, the problem of stack trace extraction from text arises, since users frequently include them in manually created bug reports. The authors present a technique of stack trace extraction and describe how to apply the TF-IDF approach for finding duplicate stack traces. Evaluations demonstrate that using stack traces in addition to textual descriptions improves the quality of bucketing. 

The study~\cite{Wu:2014:CLC:2610384.2610386} describes CrashLocator~--- a method to identify faulty functions using the crash stack information in crash reports.

The authors adapt the TF-IDF approach by introducing the notions of function frequency and inverse bucket frequency. For a given function $f$, function frequency describes its frequency of appearing in crash traces belonging to a specific bucket. Inverse bucket frequency describes the uniqueness of the function with respect to all buckets. Other factors~--- inverse average distance to crash point and function size (in lines of code) ~--- are also taken into account. In the end, the algorithm produces a ranked list of suspicious functions.

A notable idea of this approach is to expand the list of functions present in the stack trace by adding the ones that are likely to be the root cause of the crash. For this, a technique comprised of control flow analysis, backward slicing, and function change information is proposed.

Study~\cite{Campbell:2016:UET:2901739.2901766} presents a comparison of automatic crash report deduplication methods. The goal was to evaluate bucketing algorithms in industrial-scale scenarios, i.e. the ones that imply substantial (hundreds of reports per minute) rates of report arrival. Driven by these restrictions, the authors discard from consideration all algorithms that require more than $\mathcal{O}(\log n)$ comparisons per report.

The authors have considered two types of algorithms: TF-IDF-based and signature-based. The former is a classic information retrieval technique adapted for stack traces, and it is implemented by an off-the-shelf tool. The latter generate report signatures using the information contained in stack trace frames. Then, all crashes with identical signatures are assigned to a bucket identified by the signature used to create it. The results of the evaluation demonstrate the superiority of the information retrieval methods.

\newcommand{\rcl}[1]{\rotatebox[origin=rigin=c]{90}{#1}}

\begin{table*}
\caption{An overview of pairwise similarity based crash report triaging systems}
\label{tbl:classification}
\begin{center}
\begin{tabular}{ | r | c | c | c | c |c | c | p{30mm} | p{58mm} |}
\hline
\pbox{25mm}{\vspace{1.2cm}Study\vspace{-1.2cm}} & \pbox{15mm}{\vspace{1.2cm}Year\vspace{-1.2cm}} & \multicolumn{3}{ |c| }{Similarity Method} & \multicolumn{3}{ |c| }{System Aspects} & \pbox{4cm}{\vspace{1.2cm}Details\vspace{-1.2cm}} \\
\cline{3-8}
& & \rcl{signatures} & \rcl{edit~~~~~~~{}} \rcl{distance~~{}} & \rcl{TF-IDF~~{}} & \rcl{rec.~~~~~~{}} \rcl{elim.~~~~~{}} & \rcl{uninf.~~~~{}} \rcl{elim.~~~~~{}} & \pbox{4cm}{\vspace{0.9cm}indexing\vspace{-0.9cm}} & \\

\hline

Brodie et al.~\cite{brodie} & 2005 & \texttimes & \texttimes & \texttimes & \checkmark & \checkmark & Hash of Top-$K$ function names. & An adaptation of biological sequence searching algorithm. \\ \hline

Modani et al.~\cite{modani} & 2007 & \texttimes & \checkmark & \texttimes & \checkmark & \checkmark & Hash of Top-$K$ function names; inverted index function name $\longrightarrow$ stack trace. & A comparison of edit distance, prefix match and LCS approaches. \\ \hline

Bartz et al.~\cite{bartz} & 2008 & \texttimes & \checkmark & \texttimes & \texttimes & \texttimes & \texttimes & Failure similarity classifier that takes custom edit distance between callstacks as one of the parameters. \\ \hline

Dhaliwal et al.~\cite{dhaliwal} & 2011 & \checkmark & \checkmark & \texttimes & \texttimes & \texttimes & \texttimes & Two-level grouping scheme with Levenshtein distance on the second level. \\ \hline

Kim et al.~\cite{5958261} & 2011 & \texttimes & \texttimes & \texttimes & \texttimes & \texttimes & \texttimes & An adaptation of graph similarity measure. \\ \hline

Dang et al.~\cite{dang} & 2012 & \texttimes & \checkmark & \texttimes & \checkmark & \checkmark & \texttimes & A custom stack trace similarity measure and agglomerative hierarchical clustering. \\ \hline

Wang et al.~\cite{Wang:2013:IBL:2487085.2487135}& 2013 & \checkmark & \texttimes & \texttimes & \texttimes & \texttimes & \texttimes & Signatures and an adaptation of closed frequent itemset mining.\\ \hline

Lerch and Mezini~\cite{Lerch:2013:FDY:2495256.2495763} & 2013 & \texttimes & \texttimes & \checkmark & \texttimes & \texttimes & \texttimes & Combining stack traces with textual descriptions. \\ \hline

Wu et al.~\cite{Wu:2014:CLC:2610384.2610386} & 2014 & \texttimes & \texttimes & \checkmark & \checkmark & \checkmark & \texttimes & Stack trace expansion via static analysis of source code. \\ \hline

Campbell et al.~\cite{Campbell:2016:UET:2901739.2901766} & 2016 & \checkmark & \texttimes & \checkmark & \texttimes & \texttimes & Built-in in ElasticSearch & A comparison of TF-IDF and signature methods. \\ \hline
\end{tabular}
\end{center}
\end{table*}
\end{comment}


==> pseudocode.tex <==

\iftrue

\SetInd{0.125em}{0.75em}
\begin{algorithm}[h]~\label{alg:eliminate_recursion}
\caption{Recursion elimination}
\LinesNumbered
\DontPrintSemicolon

\SetKwData{Nil}{nil}

\KwIn{$ST = f_0,\ldots,f_{N-1}$ --- stack trace}
\KwOut{$ST$ --- stack trace with recursion eliminated}

$i \gets 0$

\While{$i < N$}{
	$P \gets \pi(f_i,\ldots,f_{N-1})$
	    \mbox{\hspace{1cm}//~$\pi$ is the prefix function~\cite{Knuth1977};
	          $P = p_0,\ldots, p_{\#P - 1}$.}

	\For{$j \gets \#P-1,\ldots, 1$}{
		\If{$ p_j \ne 0 \wedge (j + 1 = 0 \mod j + 1 - p_j)$}{
			remove $f_i,\ldots,f_{i + p_j - 1}$ from $ST$

%			$i \gets 0$ //~to be incremented on line 9

			\textbf{break for}
		}
	}

	\textbf{increment} $i$
}
\end{algorithm}

\fi


\iffalse

\floatname{algorithm}{Procedure}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}
  \caption{Finding last index of max repetitive frames from the beginning}
  \label{alg:find_head_recursion}
  \begin{algorithmic}[1]
    \REQUIRE $\mathit{frames}$
    \STATE $\pi$ $\gets$ the prefix function for $\mathit{frames}$
    \STATE $N$ $\gets$ $\mathit{frames}$ length
    \FOR{$i \gets$ $\pi$ reversed indices}
        \IF{$N - i \equiv 0 \mod N - i - \pi[i]$}
            \IF{$\pi[i] \neq 0$}
                \RETURN $i$
            \ENDIF
        \ENDIF
    \ENDFOR
    \RETURN $-1$
  \end{algorithmic}
\end{algorithm}

\begin{algorithm}
  \caption{Elimiate recursion}
  \label{alg:eliminate_recursion}
  \begin{algorithmic}[1]
    \REQUIRE $\mathit{frames}$
    \STATE $i \gets 0$
    \WHILE{$i <$ $\mathit{frames}$ length}
        \STATE $N \gets$ $\mathit{frames}$ length
        \STATE $j \gets$ Procedure \ref{alg:find_head_recursion} for $\mathit{frames}[i \tdots N]$
        \IF{$j \neq -1$}
            \STATE $\mathit{frames} \gets$ $\mathit{frames}[0 \tdots i]$ concatenate $\mathit{frames}[j \tdots N]$
        \ENDIF
        \STATE $i \gets i + 1$
    \ENDWHILE
  \end{algorithmic}
\end{algorithm}

\fi

\endinput


==> results.tex <==

\subsection{Similarity}

\begin{table}
    \begin{center}
        \begin{tabular}{| l | r |}
        \hline
        \textbf{Similarity approach}  & \textbf{ROC AUC} \\ \hline
        Prefix Match & $0.729 \pm 0.128$  \\ \hline
        Cosine similarity & $0.855 \pm 0.068$ \\ \hline
        Levenshtein without any heuristic & $0.638 \pm 0.126$ \\ \hline
        Levenshtein with all heuristics & $0.918 \pm 0.055$  \\ \hline
        Levenshtein without recursion removal & $0.909 \pm 0.049$  \\ \hline
        Levenshtein without position weight & $0.896 \pm 0.055$ \\ \hline
        Levenshtein without frames weight restriction & $0.894 \pm 0.069$ \\ \hline
        Levenshtein without frame weight & $0.888 \pm 0.073$ \\ \hline
        \end{tabular}
    \end{center}
    \caption{Similarity ROC AUC}\label{tab:similarity}
\end{table}

We evaluated performance for different algorithm families: Levenshtein distance, prefix match, cosine similarity with TF-IDF weights.
For Levenshtein distance there are modifications depending on whether or not heuristics were used.
Heuristics include components from frame weight described in \ref{sub:similarity} and recursion removal as part of stacktrace preprocessing described in \ref{sub:recursion}.
Cosine similarity with TF-IDF weights was computed as in \cite{lerch}.
Results are given in Table \ref{tab:similarity}.

It can be seen seen that Levenstein distance based similarity with all heurustics has significantly better result than basic Levenstein distance, as well as cosin similarity and prefix match.
Position weight, frame weight and frames weight restrictions have approximetly same contribution.
Recursion removal has less influnce, but should be noted that it's effect depends on stacktraces with recursion count.

% стектрейс зависит от количества их в выборке

% \subsection{Assignation}

% \begin{table}
%     \begin{center}
%         \begin{tabular}{| l | r | r |}
%         \hline
%         \textbf{Features group} & \textbf{AUC for group} & \textbf{AUC for all without group} \\ \hline
%         All & 0.123 &  \\ \hline
%         Time & 0.123 & 0.123 \\ \hline
%         Tf-Idf & 0.123 & 0.123 \\ \hline
%         History & 0.123 & 0.123 \\ \hline
%         Others & 0.123 & 0.123 \\ \hline
%         \end{tabular}
%     \end{center}
%     \caption{Assignation AUC}\label{tab:a}
% \end{table}


==> stacktrace.tex <==

% Stacktraces in different environments like: JVM, .NET or even c++.
All the products that we consider are mostly written in Java and Kotlin. 
They use Java Virtual Machine as platform and software problems are regulary presented as exceptions. 
Fortunately, exceptions in JVM contain stacktrace which describe program state at the time of error. 
Example [fig].

All exceptions in Java have same format [fig]. 
An exception composed from: class of exception, message and call stack functions (frames). 
Frames contain method name, file name and line number where call occurred. 
Optionally, exception may contain another nested exception. 

% There are frames that relate to loging functions or library functions.
% We don't consider them somehow differently.
% Recognizing useless of this frames we leave opportunity to decrease their influence to models themselves.
% some figure with functions like logger, execute...

We can pay attention to congeniality between stacktrace and string.
Truly, like as string is an ordered sequence of letters, so stacktrace is an ordered sequence of frames.
It allows us to use string algorithms in stacktrace processing.
The same way stactraces set can be considered as text corpus where information retrieval techniques can be used.

% most important frames at the top[ref]

==> threats.tex <==
\label{sec:validity}

We have identified the following threats to validity for our study:

\begin{itemize}
	\item \textbf{Subject selection bias.} In our study, we only use JetBrains product data. Open source projects or projects of other companies may have different initial data. Therefore, experiments run on other data may yield different results. However, some of our results are corroborated by studies that examine the same subject~\cite{dang,dhaliwal}.
	
	\item \textbf{Significant stream of reports.} Our approach is intended for software products that have a large user base and thus generate a large number of reports daily. If this is not true, our approach may not be optimal or may not be needed at all. In some cases, manual report triaging could be better.
	
\end{itemize}



